A Comparison of Few-Shot Learning Methods for Underwater Optical and Sonar Image Classification

Deep convolutional neural networks generally perform well in underwater object recognition tasks on both optical and sonar images. Many such methods require hundreds, if not thousands, of images per class to generalize well to unseen examples. However, obtaining and labeling sufficiently large volumes of data can be relatively costly and time-consuming, especially when observing rare objects or performing real-time operations. Few-Shot Learning (FSL) efforts have produced many promising methods to deal with low data availability. However, little attention has been given in the underwater domain, where the style of images poses additional challenges for object recognition algorithms. To the best of our knowledge, this is the first paper to evaluate and compare several supervised and semi-supervised Few-Shot Learning (FSL) methods using underwater optical and side-scan sonar imagery. Our results show that FSL methods offer a significant advantage over the traditional transfer learning methods that fine-tune pre-trained models. We hope that our work will help apply FSL to autonomous underwater systems and expand their learning capabilities.

==> future_work.tex <==
In the full paper, we will: 1) provide additional details of algorithms and present a full breakdown of results, 2) show that pre-meta-training can be a valuable training approach to significantly improve performance, 3) discuss the challenges faced by state-of-the-art FSL methods in real-world scenarios and how we hope to address these in our future work.

==> navigation.tex <==
\subsection{Navigation}\label{sec:navigation}
Navigation is concerned with finding the global coordinates of a robot. This is in contrast to the localization problem which is concerned in finding the position of the robot in relation to the local environment (more about this in the next section). A survey study on navigation \cite{paull2014auv} lists three ways in which underwater navigation can be achieved: (i) through dead-reckoning and use of inertial measuring unit to work out how far the vehicle moved based on time and speed of travel, (ii) by measuring the time of flight of acoustic signals with dedicated communication buoys or ships floating on/near the water surface and using triangulation, and (iii) by recognizing geophysical features in environment (such as geomagnetic data, bathymetry, rock formation, etc).
